Online Active Regression

Active regression considers a linear regression problem where the learner receives a large number of data points but can only observe a small number of labels. Since online algorithms can deal with incremental training data and take advantage of low computational cost, we consider an online extension of the active regression problem: the learner receives data points one by one and immediately decides whether it should collect the corresponding labels. The goal is to efficiently maintain the regression of received data points with a small budget of label queries. We propose novel algorithms for this problem under $\ell_p$ loss where $p\in[1,2]$. To achieve a $(1+\epsilon)$-approximate solution, our proposed algorithms only require $\tilde{\mathcal{O}}(\epsilon^{-1} d \log(n\kappa))$ queries of labels, where $n$ is the number of data points and $\kappa$ is a quantity, called the condition number, of the data points. The numerical results verify our theoretical results and show that our methods have comparable performance with offline active regression algorithms.

==> full_ell_p_alg.tex <==
\section{Algorithm for $p\in [1,2)$} \label{sec:full_ell_p_alg}

Algorithm~\ref{alg:p-online-active-regression} is the online active regression for the $\ell_p$ loss that maintains the solution for all intermediate steps.

\begin{algorithm}[!ht]
\caption{Online Active Regression for $p\in(1,2)$}
\label{alg:p-online-active-regression}
\textbf{Initialize:} Let $\tilde{A}^{(d)}, \tilde{A}_1^{(d)}, \tilde{A}_2^{(d)}, \tilde{A}_3^{(d)}$ be the first $d$ rows of $A$ and $\tilde{b}^{(d)},  \tilde{b}_2^{(d)}, \tilde{b}_3^{(d)}$ be the first $d$ rows of $b$. Let $x_{c}^{(d)} = \Call{Reg}{\tilde{A}^{(d)}, \tilde{b}^{(d)}, p}$, $\tilde{z}_{2}^{(d)}= \tilde{z}_{3}^{(d)}= \tilde{b}^{(d)}- \tilde{A}^{(d)}x_{c}^{(d)}$, $\hat{x}_{c}^{(d)} = \Call{Reg}{\tilde{A}_{2}^{(d)}, \tilde{z}_{2}^{(d)}, p}$ and $\bar{x}'_{d} = \Call{Reg}{\tilde{A}_{3}^{(d)}, \tilde{z}_{3}^{(d)}- \tilde{A}_{3}^{(d)}\hat{x}_{c}^{(d)}, p}$. 
\begin{algorithmic}[1]
\State $\beta \gets (3\log d)/\eps^2$
\State $\beta_{1} \gets d/\eps^4$
\State $\beta_{2} \gets (3\log d)/\eps^2$
\State $\beta_{3} \gets \log^2 d\log(d/\eps) /\eps^{2p+5}$
\State retain the first $d$ rows of $A$
\While{there is an additional row $a_t$}
    \State $\tilde{w}_t \gets w_t(A^{(t)})$ \label{alg:line:online_lewis_appendix}
    \State $p_t = \min\{\beta\tilde{w}^{(t)}, 1\}$
    \State $(x_{c}^{(t)},\tilde{A}^{(t)}, \tilde{b}^{(t)}) \gets 
    \Call{SampleQuery}{a_t, \tilde{A}^{(t-1)}, \tilde{b}^{(t-1)}, \NULL, p_t, p}$
    \State $\tilde{w}_{1,t} \gets w_{\last}(\tilde{A}^{(t)})$ \label{alg:line:online_lewis1_appendix}
    \State $p_{1,t} = \min\{\beta_1 \tilde{w}_{1,t}, 1 \}$
    \State Sample $a_t$ with probability $p_{1,t}$
    \If{$a_t$ is sampled}
        \State $(\tilde{A}_{1}^{(t)}, \tilde{b}_{1}^{(t)}) \gets (\tilde{A}_{1}^{(t-1)} \circ a_t^{\top} p_{1,t}^{-1/p}, \tilde{b}_{1}^{(t-1)} \circ b_t p_{1,t}^{-1/p})$
        %\State $\tilde{z}_{1}^{(t)} \gets \tilde{b}_{1}^{(t)} - \tilde{A}_{1}^{(t)} x_c^{(t)}$
        \State $\tilde{w}_{2,t} \gets w_{\last}(\tilde{A}_1^{(t)}) $ \label{alg:line:online_lewis2_appendix}
        \State $p_{2,t} \gets \min \{ \beta_2 \tilde{w}_{2,t}, 1 \}$
        \State $(\hat{x}_{c}^{(t)}, \tilde{A}_{2}^{(t)}, \tilde{b}_{2}^{(t)}) \gets 
        \Call{SampleQuery}{a_{t} p_{2,t}^{-1/p}, \tilde{A}_{2}^{(t-1)}, \tilde{b}_{2}^{(t-1)}, \NULL, p_{2,t}, p}$
        \State $\tilde{w}_{3,t} \gets w_{\last}(\tilde{A}_2^{(t)})$ \label{alg:line:online_lewis3_appendix}
        \State $p_{3,t} \gets \min \{ \beta_3 \tilde{w}_{3,t}, 1 \}$
        \State $(\hat{x}_{c}^{(t)}, \tilde{A}_{3}^{(t)}, \tilde{b}_{3}^{(t)}) \gets 
        \Call{SampleQuery}{a_{t} p_{3,t}^{-1/p}, \tilde{A}_{3}^{(t-1)},
        \tilde{z}_{3}^{(t-1)}, \hat{x}_{c}^{(t)}, p_{3,t}, p}$
        \State $\bar{x}^{(t)} \gets \hat{x}_{c}^{(t)} + \bar{x}^{'(t)}$
        \State $\tilde{x}^{(t)} \gets x_c^{(t)}+\bar{x}^{(t)}$
    \Else
        \State $(\tilde{A}_{1}^{(t)}, \tilde{b}_{1}^{(t)}) \gets (\tilde{A}_{1}^{(t-1)}, \tilde{b}_{1}^{(t-1)})$
    \EndIf
\EndWhile
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[!ht]
\caption{$\Call{SampleQuery}{a_t, \tilde{A}^{(t-1)}, \tilde{b}^{(t-1)}, \hat{x}_{c}^{(t)}, p_t, p,\chi}$ in Algorithm~\ref{alg:p-online-active-regression}}
\label{alg:p-sample-query}
\begin{algorithmic}[1]
\State Sample $a_t$ with probability $p_t$
\If{$a_t$ is sampled}
    \State $\tilde{A}^{(t)} \gets \tilde{A}^{(t-1)} \circ a_t^{\top} p_t^{-1/p}$
    \State \textbf{Query} $b_t$
    \If{$\chi = 1$}
        \State $\tilde{b}^{(t)}\gets \tilde{b}^{(t-1)} \circ b_t p_t^{-1/p}$
    \Else
        \State $\tilde{b}^{(t)}\gets \tilde{b}^{(t-1)} \circ b_t p_{1,t}^{-1/p} p_t^{-1/p}$
        \State $\tilde{z}^{(t)}= \tilde{b}^{(t)}-\tilde{A}^{(t)}\hat{x}_c^{(t)}$
    \EndIf
\Else 
    \State $(\tilde{A}^{(t)}, \tilde{b}^{(t)}) \gets (\tilde{A}^{(t-1)}, \tilde{b}^{(t-1)})$
\EndIf
\If{$\chi=1$ is}
    \State $x^{(t)} \gets \Call{Reg}{\tilde{A}^{(t)}, \tilde{b}^{(t)}, p}$
\ElsIf{$\hat{x}_c^{(t)} = \NULL$}
    \State$\Call{Reg}{\tilde{A}^{(t)}, \tilde{z}^{(t)}, p}$
    \Else
        \State $\Call{Reg}{\tilde{A}^{(t)}, \tilde{b}^{(t)} - \tilde{A}^{(t)} \hat{x}_c^{(t)}, p}$
\EndIf
\State \Return $(x^{(t)},\tilde{A}^{(t)}, \tilde{b}^{(t)})$
\end{algorithmic}
\end{algorithm}

==> preserve.tex <==
It's remained to prove the sampling scheme preserves the norm of $Ax-z$ for all $x$ in $\cN_\eps$. From here, we use two different net construction methods to prove it. The first way is to use the entropy estimate and net construction in\cite{BLM}. This finer net construction allows us to remove the dependence of $\beta$ on $d$ when the inequality is taken over $\cN_\eps$. The second way is to use the Freedman inequality \cite{trp} about scalar martingale, which is relatively easy but will cause the dependence of query complexity on d rise to $d^2$. At last, we will combine these two methods to obtain the result in our main theorem.

Now, we show the first way of proving the inequality to hold for all $x\in\R^d$ with $\norm{Ax}_2\leq1$.

\begin{lemma}
Let $SA$ be the sampled matrix, z be the same as the setting ..and $\beta=\frac{\log(n)}{\eps^6}$. With high probability, for any $x\in\R^d$ with $\norm{Ax}_p\leq 1$, $\Abs{\norm{SA x-Sz}_p^p-\norm{Ax-z}_p^p}=\cO(\eps)\OPT^p$.
\end{lemma}

We use a proof similar to Lemma 3.7 in\cite{m2a}. But we provide a more tighter bound than their result in the dependence of query complexity on $\eps$ and reduce the power from $\min(p+7,2p+5)$ to $\min(p+4,2p+2)$.
The detailed proof is in the appendix.

Before proving the lemma 2, we first introduce some 

\begin{lemma}\label{lem:d^2}
Let $SA$ be the sampled matrix, z be the same as the setting ..and $\beta=\frac{d}{\eps^4}$. With high probability, for any $x\in\R^d$ with $\norm{Ax}_p\leq 1$, $\Abs{\norm{SA x-Sz}_p^p-\norm{Ax-z}_p^p}=\cO(\eps)\OPT^p$.
\end{lemma}

\begin{proof}
Here, we use the matrix Freedman inequality. Let $Y_i=\norm{\tilde{A}_ix-\tilde{z}_i}_2^2-\norm{A_ix-z_i}_2^2$, $Y_0=0$ and $X_i = Y_i-Y_{i-1}$. Then, $\abs{X_i}$ is uniformly bounded. 
\begin{align*}
    \abs{X_i}&=\Abs{\Norm{\frac{\mathbbm{1}_{i}}{\sqrt{p_i}}(a_ix-z_i)}_2^2-\norm{a_ix-z_i}_2^2}\\
    &\leq\frac{1}{p_i}\cdot\norm{a_ix-z_i}_2^2.
\end{align*}
Here, we use the definition of $\mathcal{B}$ in... If $i\in\mathcal{B}$, $\bar{z}_i=0$, then, by Cauchy-Schwarz inequality, we have $\norm{a_ix}_2^2\leq w_i^2\norm{Ax}_2^2=w_i \cO(\text{OPT}^2)$. Otherwise, $\norm{a_ix-z_i}_2^2\leq(\frac{1}{\epsilon}+1)^2 w_i^2 \cO(\OPT)^2$. Hence, since $p_i=\min(\beta w_i,1)$, we have $\norm{Y_i-Y_{i-1}}\leq\frac{1}{\beta\epsilon^2}\cO(\OPT^2)$. $\E(X_i^2|Y_i,\dots,Y_1)$ is denoted by $\E_{i-1}X_i^2$ .
\begin{align*}
    \E_{i-1}X_i^2&=\E\left(\norm{\frac{1}{\sqrt{p_i}}(a_ix-z_i)}_2^2-\norm{a_ix-z_i}_2^2\right)^2\\
    &=\E(\frac{1}{p_i}-1)^2\norm{a_ix-z_i}_2^4\\
    &=(\frac{1}{p_i}-1)\norm{a_ix-z_i}_2^4\\
    &\leq\frac{w_i}{p_i}(\frac{1}{\epsilon}+1)^2\cO(\OPT^2)\norm{a_ix-z_i}_2^2\\
    &\leq\frac{1}{\beta\epsilon^2}\cO(\OPT^2)\norm{a_ix-z_i}_2^2.
\end{align*}

Therefore, $\sum_{i=1}^{i=n}\E_{i-1}X_i^2\leq\frac{1}{\beta\epsilon^2}\cO(\OPT^2)\cdot\sum_{i=1}^{i=n}\norm{a_ix-z_i}_2^2$.
Since $\norm{Ax}_2^2=\cO(\OPT^2)$ and $\norm{z}_2^2=\cO(\OPT^2)$, we can get $\sum_{i=1}^{i=n}\E_{i-1}X_i^2\leq\frac{1}{\beta\epsilon^2}\cO(\OPT^4)$.

Then, by the matrix Freedman inequality \cite{trp} and $\beta=\frac{d\log(\frac{1}{\delta})}{\epsilon^4}$, it follows that
\begin{align*}
  \Pr(\norm{Y_n}\geq\cO(\epsilon)\OPT^2)&\leq\exp\left\{\frac{-\epsilon^2\cO(\OPT^4)}{\frac{1}{\beta\epsilon^4}\cO(\OPT^4)+\frac{\cO(\OPT^4)}{3\beta\epsilon}}\right\}\\
  &\leq\exp\{\frac{-\beta\epsilon^4}{2}\},
\end{align*}

which implies that with probability at least $1-\frac{\delta}{2^d}$, $\Abs{\norm{\tilde{A}x-\tilde{z}}_2^2-\norm{Ax-z}_2^2}\leq\cO(\epsilon)\text{OPT}^2$, for a fixed $x\in\R^d$.

To simplify the writing, without loss of generality, we assume $\OPT=1$ in the next proof.  Now we apply a union bound over an $\epsilon$-net $\mathcal{N}$ of the ball $\mathbf{B} = \{x\in\R^d|\,\norm{Ax-z}_2^2=1)\}$. %Construct the $\epsilon$-net by a greedy process.  
Note that there are at most $(\frac{3}{\epsilon})^d$ points in the $\epsilon$-net. Applying a union bound over the net, $\Abs{\norm{\tilde{A}x-\tilde{z}}_2^2-\norm{Ax-z}_2^2}\leq\cO(\epsilon)$ holds for each point in $\mathcal{N}$ with probability at least $1-\delta$. 

For any $x\in\R^d$ with $\norm{Ax}_2^2 =1$, by the definition of $\epsilon$-net, there exists a vector $y\in\mathcal{N}$ such that $\norm{Ax-Ay}_2\leq\epsilon$. We have proved that $\tilde{A}^\top A$ is a good spectral approximation of$A^\top A$, so $\norm{\tilde{A}x-\tilde{A}y}_2\leq\cO(\epsilon)$ Hence, we have
\begin{align*}
\Abs{\norm{\tilde{A}x-\tilde{z}}_2-\norm{Ax-z}_2}&\leq\Abs{\norm{\tilde{A}y-\tilde{z}}_2-\norm{Ay-z}_2}+\norm{\tilde{A}x-\tilde{A}y}_2+\norm{Ax-Ay}_2\\
&\leq\cO(\epsilon)+\cO(\epsilon)+\epsilon,\end{align*}
which completes our proof.
\end{proof}
